Irreducibility of the Wysiwyg representations of Thompson's groups

We prove irreducibility and mutual inequivalence for certain unitary representations of R. Thompson's groups F and T.

==> attach <==
#FIG 3.2  Produced by xfig version 3.2.5b
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 1200 2400 6000 7200 10800 2400
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3000 2400 6900 6300
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4800 2400 7800 5400
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6600 2400 8700 4500
2 1 1 6 0 7 50 -1 -1 14.000 0 0 -1 0 0 2
	 6600 2400 10800 2400
4 0 0 50 -1 3 100 0.0000 4 750 645 8475 3600 s\001

